Finite-Time Convergence and Sample Complexity of Actor-Critic Multi-Objective Reinforcement Learning

Reinforcement learning with multiple, potentially conflicting objectives is pervasive in real-world applications, while this problem remains theoretically under-explored. This paper tackles the multi-objective reinforcement learning (MORL) problem and introduces an innovative actor-critic algorithm named MOAC which finds a policy by iteratively making trade-offs among conflicting reward signals. Notably, we provide the first analysis of finite-time Pareto-stationary convergence and corresponding sample complexity in both discounted and average reward settings. Our approach has two salient features: (a) MOAC mitigates the cumulative estimation bias resulting from finding an optimal common gradient descent direction out of stochastic samples. This enables provable convergence rate and sample complexity guarantees independent of the number of objectives; (b) With proper momentum coefficient, MOAC initializes the weights of individual policy gradients using samples from the environment, instead of manual initialization. This enhances the practicality and robustness of our algorithm. Finally, experiments conducted on a real-world dataset validate the effectiveness of our proposed method.

==> finite_time.tex <==
\section{Theoretical Convergence Analysis}
In this section, we present the convergence results for both the critic and actor steps in Theorems~\ref{the: critic} and \ref{the: actor}, respectively. 
Due to space limitation, we relegate the proofs to the supplementary material.

\subsection{Convergence Analysis for Critic (Algorithm~\ref{alg: critic})}
For a given policy $\pi_{\theta}$, we define $b_{\pi_{\theta}}=\mathbb{E}_{s\sim d_{\theta},a\sim \pi_{\theta}}[\phi(s)(\bar{r}(s,a)-J(\theta))]$, where $\bar{r}(s,a)=\frac{1}{N}\sum_{i\in\mathcal{N}}r^{i}(s,a)$ and $J(\theta)$ are as defined in (\ref{eq: obj}). 
For all agents, the optimal solution \citep{WuZhaXu_20}, \citep{QiuYanYe_21} of this critic learning is $w^{*}_{\theta}=-A^{-1}_{\pi_{\theta}}b_{\pi_{\theta}}$ 
, where $A_{\pi_{\theta}}$ is defined as in (\ref{eq: A_pi}). 
The invertiblity of $A_{\pi_{\theta}}$ is due to the Assumptions~\ref{ass: con_diff_dis} and \ref{ass: fea} (see more details in \citep{QiuYanYe_21,TsiVan_99}).
Then, the convergence of the critic step is summarized as follows:
\begin{theorem}[Convergence and Sample Complexity of the Critic] 
Suppose that Assumptions \ref{ass: con_diff_dis}-\ref{ass: lam} hold. 
For any given policy $\pi_{\theta}$, consider the iteration generated by Algorithm \ref{alg: critic}. 
Recall the definition of $\lambda_A$ in the Assumption \ref{ass: lam} and let $\beta<\min\{\frac{\eta^{N-1}}{2(1-\eta^{N-1})},\frac{\lambda_A}{128},\frac{4}{\lambda_A}\}$. 
It then follows that:
\begin{align}
\mathbb{E}[\sum_{i=1}^{N}||w^{i}_{K_c}-w^{*}_{\theta}||^{2}]&\le\kappa'_1N^{4}\gamma^{2K_c}+\kappa''_2N^{6}\beta^{2}+\kappa_3N^{5}\gamma^{K_c}\beta \nonumber \\ &\quad+2N(1-\frac{\lambda_A}{8}\beta)^{K_c}||\bar{w}_0-w^{*}_{\theta}||^{2}_2+\frac{\kappa_4}{M}N, 
\label{eq: critic}
\end{align}
where $\gamma:=(1-\eta^{N-1})\cdot(1+2\beta)<1$ and $\kappa'_1,\kappa''_2,\kappa_3,\kappa_4$ are positive constants.
If we further let \textcolor{red}{$K_c\ge\max\{\frac{8}{\beta\lambda_A}\ln\frac{10N||\bar{w}_0-w^{*}_{\theta}||^{2}_2}{\epsilon},\frac{1}{2}\log_{\frac{1}{\gamma}}\frac{5\kappa'_1N^{4}}{\epsilon}\}$}, $\beta\le\min\{\frac{1}{N^{3}}\sqrt{\frac{\epsilon}{6\kappa''_2}},\frac{\eta^{N-1}}{2(1-\eta^{N-1})},\frac{\lambda_A}{128},\frac{4}{\lambda_A}\}$ and
$M\ge \frac{6\kappa_4N}{\epsilon}$, then for a small $\epsilon>0$, we have $\mathbb{E}[\sum_{i=1}^{N}||w^{i}_{K_c}-w^{*}_{\theta}||^{2}]\le\epsilon$ for all $i\in\mathcal{N}$ with total sample complexity given by $K_cM=\mathcal{O}(\frac{N}{\epsilon\textcolor{red}{\sqrt{\epsilon}}}\log(\frac{N}{\epsilon}))$.
\label{the: critic}
\end{theorem}
Theorem~\ref{the: critic} establishes a convergence result for the policy evaluation of a given policy $\pi_{\theta}$. We can see that our constant step-size batch-sampled critic process can achieve the same complexity of $\tilde{\mathcal{O}}(\epsilon^{-1})$ order-wise as the TD(0) learning in \cite{DoaMagRom_19}, where  diminishing step-sizes were used. On the other hand, in the single agent average reward setting of \cite{QiuYanYe_21}, there exists a non-vanishing error term in their critic convergence. In contrast, with proper choices of iteration number $K_c$ and batch size $M$, our mean-square error can be arbitrarily small.
%The system size $N$ appears in the latter two non-vanishing terms of \eqref{eq: critic}, which suggest that the convergence error neighborhood linearly depends on the network size.

%is due to the use of triangle inequality. This might be improved with better techniques, which shall be in the future work.


\subsection{Convergence Analysis for Actor-Critic Algorithm (Algorithm~\ref{alg: actor})}
Define the approximation error introduced by using linear approximation in the critic step, $\xi^{\text{critic}}_{\text{approx}}=\max_{\theta\in\mathbb{R}^{\sum_{i\in\mathcal{N}}m^{i}}} \mathbb{E}_{s\sim d_{\theta}}[|V_{\pi_{\theta}}(s)-V_{w^{*}_{\pi_{\theta}}}(s)|^{2}]$. 
For a given policy $\pi_{\theta}$, this error represents the gap between ground truth value function under such policy and the value function obtained by the best possible linear approximation. Such an error term is standard in the literature where linear approximations are adopted \citep{QiuYanYe_21,XuWanLia_20}. 
Let $R_{w}$, defined in Lemma \ref{lem: w_opt_bou}, be an upper bound on $||w_{\theta}||$ for all policy parameter $\theta$. 
\begin{theorem}[Overall Convergence Rate and Sample Complexity] \label{thm:actor}
Suppose that Assumption \ref{ass: con_diff_dis}-\ref{ass: Lip_bou} hold. Consider the actor-critic algorithm in Algorithm \ref{alg: actor}. Let step-size $\alpha=\frac{1}{4L_J}$. 
It then holds that:
\begin{align}
\mathbb{E}[||\nabla_{\theta} J(\theta_{\tilde{T}})||^{2}] \le &\frac{16L_J r_{\max}}{T}+72N\frac{\sum_{t=1}^{T}\sum_{i=1}^{N}||w^{i}_t-w^{*}_{\theta_t}||^{2}}{T}+18\kappa_3N^{3}(1-\eta^{N-1})^{2t_{\text{gossip}}} \nonumber \\
&+72\xi^{\text{critic}}_{\text{approx}}+288\frac{(r_{\max}+R_{w})^{2}[1+(2\kappa-1)\rho]}{B(1-\rho)}N, 
\label{eq: actor}
\end{align}
where $\kappa_3$ is a positive constant.
Furthermore, let $T\ge\frac{64L_J r_{\max}}{\epsilon}$, $B\ge576\frac{(r_{\max}+2R_{w})^{2}[1+(2\kappa-1)\rho]}{(1-\rho)}\frac{N}{\epsilon}$ and the communication round among the agents $t_{\text{gossip}}\ge\frac{1}{2}\log_{(1-\eta^{N-1})^{-1}}\frac{64\kappa_3 N^{3}}{\epsilon}$. Suppose for the same setting as in Theorem 1 holds so that $\mathbb{E}[\sum_{i=1}^{N}||w^{i}_{K_c}-w^{*}_{\theta}||^{2}]\le\frac{\epsilon}{288N}$ for all $0\le t\le T$, then we have 
$\mathbb{E}[||\nabla_{\theta} J(\theta_t)||^{2}] \le \epsilon+\mathcal{O}(\xi^{\text{critic}}_{\text{approx}}),$
with a total complexity of $(B+MK_c)T=\mathcal{O}(\frac{N^{2}}{\epsilon^{2}\sqrt{\epsilon}}\log(\frac{N}{\epsilon}))$. And the communication complexity is $(K_c+t_{\text{gossip}})T=\mathcal{O}(\frac{1}{\epsilon\textcolor{red}{\sqrt{\epsilon}}}\log(\frac{N}{\epsilon}))$.
\label{the: actor}
\end{theorem}
Theorem~\ref{the: actor} concludes the overall sample complexity of our proposed actor-critic algorithm. The sample complexity of $\mathcal{O}(\epsilon^{-2}\log(\epsilon^{-1}))$ matches the state-of-the-art single-agent actor-critic RL by \cite{XuWanLia_20} and the discounted MARL by \cite{CheZhoChe_21}. 
%The $N$ that appears both in the second and the last non-vanishing terms of \eqref{eq: actor} is due to the decomposition of $N$ terms, see more dtailed discussions in \ref{subsec: actor}.

We note that the overall communication complexity also matches that of \citep{CheZhoChe_21} in the discounted reward setting. 
%due to the use of similar techniques. 
However, our work is still an improvement compared to the classical MARL in \cite{ZhaYanLiu_18} for the average reward setting.
Specifically, 
\cite{ZhaYanLiu_18} needed a communication round after each sampling.
By contrast, in this paper, we only need a communication round per $\mathcal{O}(\epsilon^{-1})$ sampling. 
This is thanks to the use of batch sampling in the actor step. Also because of the batch sampling, we are able to use a constant step-size for both actor and critic steps. 
Here, the overall communication cost is measured by the number of communication rounds rather than the size of bits transmitted over the network. We follow the standard definition of communication complexity in the literature, which is widely adopted in the literature, see  \citep{CheGiaSun_18} \citep{ZhaLiuZhu_19}.
However, we note that $t_{\text{gossip}}$, actor step batch size $B$ and critic iteration rounds $K_c$, scale with $\mathcal{O}(\log 1/\epsilon)$, $\mathcal{O}(1/\epsilon)$ and $\mathcal{O}(\log 1/\epsilon)$ respectively as indicated in the Theorem \ref{the: actor} and \ref{the: critic}.
The amount of information (in terms of bits) is 
$(K_c NK+BNt_{\text{gossip}})T=\mathcal{O}(\frac{N}{\epsilon^{2}\textcolor{red}{\sqrt{\epsilon}}}\log \frac{N}{\epsilon})$.






==> introduction_v1.tex <==
\section{Introduction}
Reinforcement learning has attracted increasing attention from both academia and industry, due to its nature of dynamically mapping situations to actions with no dependency on labeled data.
So far, most reinforcement learning literature focus on single reward signal optimization \citep{yang2019provably,XuWanLia_20,afsar2022reinforcement,ma2020off}, while realistic scenarios often require finding one policy that optimizes multiple, potentially conflicting reward signals, which is so-called multi-objective reinforcement learning (MORL).
For example, e-commerce services rank products by taking into account preferences of different user groups, some of which prefer faster delivery, while others may prefer lower price even with slower delivery. 
Formally, MORL with parameterized policy can be formulated as follows:
\begin{equation}
    \max_{\bm{\theta}\in\mathbb{R}^{d_1}}\bm{J}(\bm{\theta}) := \left( J^1(\bm{\theta}), J^2(\bm{\theta}), \ldots, J^M(\bm{\theta}) \right)^{\top}, \nonumber
\end{equation}
where $\bm{\theta}$ is the policy parameter for policy $\pi_{\bm{\theta}}$, and $J^i(\bm{\theta})$ is the expected total reward for objective $i\in[M]$ induced by policy $\pi_{\bm{\theta}}$ (we will define two common objectives of $J^{i}(\bm{\theta})$ later in Section \ref{sec: J_def}).
In this problem, there may not always exist a common parameter that maximizes all individual objectives simultaneously.
Therefore, a natural solution is to find a Pareto optimal point for all objectives that cannot be further improved without sacrificing any individual objective.
However, similar to single-objective non-convex optimization problem, finding global optimum (or equivalently Pareto optimal in multi-objective setting) is NP-hard in general \citep{DanDvuGas_22,YanLiuLiu_23}. To obtain a meaningful solution, a concept of Pareto stationary point, which is a necessary condition for being a Pareto optimal, is proposed in many gradient based approaches \citep{Des_12,SenKol_18,YanLiuLiu_23}. In this paper, as a first step towards understanding and characterizing the finite-time convergence results and sample complexity, we focus on the convergence to Pareto stationary point.

In multi-objective optimization, multiple gradient descent algorithm (MGDA) has been developed for finding a Pareto stationary point \citep{Des_12}.
MGDA is an extension of classic gradient descent algorithm, which defines a common descent direction as a minimum $\ell_2$ norm element in the convex hull of the gradients from all individual objectives.
The convergence of MGDA and its variants have been studied under different settings of multi-objective context, including convex and non-convex objective functions \citep{liu2021stochastic,FerSheLiu_22}, decentralized data \citep{YanLiuLiu_23}, etc.
However, developing RL algorithms in multi-objective context with provable Pareto stationary convergence remains under-explored.
To find a solution to MORL, some major challenges of incorporating MGDA to RL methods are listed as follows:
\vspace{-1em}
\begin{list}{\labelitemi}{\leftmargin=1.5em \itemindent=-0.0em \itemsep=-.2em}
\item[a)] As a policy gradient method, actor-critic method learns approximations to policy and value functions in a bootstrapping manner.
This allows the incorporation of MGDA in computing a common gradient descent direction of policy parameter.
However, it is unclear whether such method can achieve Pareto stationary convergence and if so, how to characterize the finite-time convergence and sample complexity.
\item[b)] Both actor and critic update their parameters through stochastic approximations. However, applying MGDA in stochastic setting introduces cumulative estimation bias, since MGDA always finds optimal gradient weights while the gradients are obtained from sampling. Such cumulative estimation bias could lead to degraded performance in reward maximization or even non-convergence of policy parameter.
\end{list}
\vspace{-1em}

% As a trade-off, one can always transform a MORL problem to a single-objective reinforcement learning problem by pre-specifying the weights \citep{mossalam2016multi, white1980solution}, however, quantifying the weights becomes a new challenge and it remains unclear whether a learnt policy is optimal on balancing conflicting objectives.

% In multi-objective optimization (MOO), a prominent solution is to find a Pareto stationary point for all objectives that cannot be further improved without sacrificing any individual objective.
% In this context, multiple gradient descent algorithm (MGDA) has been proposed.

% Pareto stationary point is a point satisfying certain first-order necessary conditions for being Pareto optimal. To ease the understanding of the solution concepts in multi-objective context, one can compare it with the conventional single-objective optimization. In such parallel comparison, Pareto optimal point corresponds to a global optimal and Pareto stationary point can be similarly understood as stationary point as in conventional single-objective optimization.

In this paper, we overcome all the above challenges, and we summarize our contributions as follows:
% Our key contribution is that we introduce an MGDA-based actor-critic algorithm for MORL with provable Pareto-stationary convergence rate and sample complexity guarantees.
% Our major contributions are summarized as follows:
\vspace{-1em}
\begin{list}{\labelitemi}{\leftmargin=1.5em \itemindent=-0.0em \itemsep=-.2em}
\item We propose an actor-critic multi-objective reinforcement learning algorithm named \policy and provide finite-time convergence rate to Pareto Stationary point and sample complexity of $\mathcal{O}(1/\epsilon^{2})$ for a $\epsilon$-closeness Pareto stationary point, both in discounted and average reward settings. Such finite time convergence and sample complexity results are the first of its kind in MORL.
% \item By utilizing momentum approach for weight balance among individual policy gradients and selecting very common step sizes, our algorithm do not require initialization of weights for individual objective gradients. This approach not only ensures finite-time convergence and sample complexity guarantees and also enhances the practicality and robustness of our algorithm and without manually choosing weights among objectives.
\item We incorporate momentum mechanism to mitigate the cumulative estimation bias resulted from finding an optimal common gradient descent direction out of stochastic samples. One implicit advantage is that the convergence rate and sample complexity of \policy do not scale with the number of objectives. This is a sharp contrast to most related results in multi-objective optimization, where the convergence results are either linear with respect to $M$ \citep{FerSheLiu_22} or have an high-order dependency $\mathcal{O}(M^{3})$ \citep{ZhoZhaJia_22}. On the other hand, with proper momentum coefficient, \policy initializes the weights of individual policy gradients out of samples from the environment, instead of manual initialization. This enhances the practicality and robustness of our approach.
\item We conduct experiment on real-world dataset and show that the off-policy version (for fair comparison) of our method outperforms other relevant state-of-the-art methods in MORL.
\end{list}
\vspace{-1em}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> related_work.tex <==
\section{Related Work}
In this section, we provide an overview of the related work in general MOO and MORL to put our work in comparative perspectives.

\textbf{1) MGDA-based Multi-objective Optimization:}
Multi-objective optimization (MOO) \cite{Mie_99} is concerned with optimizing a set of objective functions simultaneously over a shared parameter. 
In the context of gradient based optimization, the significance of MOO is that given a gradient update direction, different objectives might have conflicting updates. That is to say, some objective functions might increase and others might decrease. To balance among the objective functions and optimize all of them, Multiple-Gradient Descent Algorithm(MGDA) \cite{Des_12}, which generalizes the widely used gradient approach, is proposed to find a Pareto stationary point. However, the convergence analysis in \cite{Des_12} is only asymptotic and later in \cite{FliVazVic_19}, it's shown that the convergence rates are the same for multi-objective optimization to their single-objective counterparts under certain assumptions.

%Multi-task optimization(MTO) is to solve a very similar problem as in MOO except that the ultimate objective function is a scalarized version of the original objective functions. In other words, a predefined weight is assigned for each original objective function and the ultimate objective function is a weighted sum of these original objective functions. Instead of optimizing over a vector objective function, MTO aims to solve a scalar objective function as in conventional optimization problem. However, a significant drawback of such an approach is to provide a set of predefined weights.

A line of recent research in various settings of machine learning problems \cite{SenKol_18,YanLiuLiu_23,FerSheLiu_22,XiaBanJi_23,ZhoZhaJia_22} utilizes MGDA or its variants to characterize the convergence rates to Pareto stationary points. However, the convergence rates in the literature do not translate into MORL as we focus on the finite time convergence and complexity in terms of sample number. Nevertheless, we do note that in these literature the convergence tends to scale with respect to the number of objectives $M$, whereas both finite-time and sample complexity results in this work are objective-dimension-free. 


\textbf{2) Multi-objective Reinforcement Learning:}
Reinforcement learning \cite{SutBar_18} is a setting where multiple reward signals can be present, e.g. online recommendation services \cite{CheDuXia_21,CaiXueZha_23} and balancing utility and fairness \cite{GeZhaYu_22}. Traditional reinforcement learning \cite{SutBar_18,KonTsi_99,XuWanLia_20,GuoHuZha_21} only focuses on scalar rewards rather than vector rewards. In an attempt to propose solution for MORL, an actor critic algorithm that utilizes deterministic policy gradient has been proposed in \cite{CheDuXia_21}. In \cite{CaiXueZha_23}, a two-stage constrained actor critic algorithm is proposed. In the formulation, all but one objective is considered as constraints, addressed in the first stage of the algorithm, and then the remaining objective is maximized as the system objective in the second stage. However, there's no finite-time convergence or sample complexity guarantees provided in either work.

Notably, multi-agent reinforcement learning(MARL) \cite{ZhaYanLiu_18,CheZhoChe_21,HaiLiuLu_22} resembles MORL from the point of multiple reward signals as each agent receives scalar rewards. However, the objective function is a weighted sum of the rewards from all agents, where uniform weight is a common choice. Similarly, a scalarized version of MORL is considered in \cite{StaKarAra_22} so that solutions of single objective can be utilized for recommender systems. Constrained (or safe) reinforcement learning \cite{WeiLiuYin_22,CaiXueZha_23} is another approach for balancing various objectives of reinforcement learning. However, there's a set of predefined constraint parameters to identify the constraint level. In comparison, the algorithm proposed in this paper is a parameter free approach.

